Inter-Particle Potentials in Non-Linear Quantum Field Theories

This research is concerned with the inter-particle potentials for few-particle bound state systems in a scalar model with a Higgs-like mediating field and QCD. The variational method, in a reformulated Hamiltonian formalism of QFT, is used to derive relativistic few particle wave equations and, consequently, the corresponding inter-particle potentials for stationary states of systems in question. The cubic and quartic contributions to the inter-particle potentials, in the non-relativistic limit, are expressed as multi-dimensional integrals. In the scalar Higgs-like model, when the mediator is massive, it is found that the non-linear terms modify the attractive Yukawa potential. In the case of QCD, the derived quark-antiquark potential is significantly affected by the non-linear terms and provides a signal of confinement.

==> abstract.tex <==
This research is concerned with the inter-particle potentials for few-particle bound state systems in a scalar model with a Higgs-like mediating field and QCD. The variational method, in a reformulated Hamiltonian formalism of QFT, is used to derive relativistic few particle wave equations and, consequently, the corresponding inter-particle potentials for stationary states of systems in question. The cubic and quartic contributions to the inter-particle potentials, in the non-relativistic limit, are expressed as multi-dimensional integrals. In the scalar Higgs-like model, when the mediator is massive, it is found that the non-linear terms modify the attractive Yukawa potential. In the case of QCD, the derived quark-antiquark potential is significantly affected by the non-linear terms and provides a signal of confinement.




==> acknowledgements.tex <==
%

I'd like to thank the following graduate students who either shared the office and/or had insightful and stimulating discussions about physics and other topics with me: Monika Aggarwal, Alain Marsman, Banafsheh Hashemi Pour, Amir Gershon, Laura Chajet, Mark Wurtz. In addition, a special thanks goes to Alexey Illarionov for his help related to programming. 

Next, I'd like to thank the members of my supervisory committee: Roman Koniuk and Randy Lewis for the useful discussions related to my research and physics in general. 

Also, I'd like to thank the graduate secretary Marlene Caplan for all the administrative support she has provided. 

Finally, I'd like to thank my supervisor Jurij Darewych for his committed assistance and patience, for the useful discussions and guidance in the research activities. 


==> dedication.tex <==
I dedicate this dissertation to my father, mother, sister and wife. 

